CD-TWINSAFE: A ROS-enabled Digital Twin for Scene Understanding and Safety Emerging V2I Technology

In this paper, the CD-TWINSAFE is introduced, a V2I-based digital twin for Autonomous Vehicles. The proposed architecture is composed of two stacks running simultaneously, an on-board driving stack that includes a stereo camera for scene understanding, and a digital twin stack that runs an Unreal Engine 5 replica of the scene viewed by the camera as well as returning safety alerts to the cockpit. The on-board stack is implemented on the vehicle side including 2 main autonomous modules; localization and perception. The position and orientation of the ego vehicle are obtained using on-board sensors. Furthermore, the perception module is responsible for processing 20-fps images from stereo camera and understands the scene through two complementary pipelines. The pipeline are working on object detection and feature extraction including object velocity, yaw and the safety metrics time-to-collision and time-headway. The collected data form the driving stack are sent to the infrastructure side through the ROS-enabled architecture in the form of custom ROS2 messages and sent over UDP links that ride a 4G modem for V2I communication. The environment is monitored via the digital twin through the shared messages which update the information of the spawned ego vehicle and detected objects based on the real-time localization and perception data. Several tests with different driving scenarios to confirm the validity and real-time response of the proposed architecture.

==> files/title.tex <==
\title{\LARGE \bf CD-TWINSAFE: A ROS-enabled Digital Twin for Scene Understanding and Safety Emerging V2I Technology}

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
\author{
\IEEEauthorblockN{
Amro Khaled\IEEEauthorrefmark{1}\IEEEauthorrefmark{2}$^{\orcidicon{0009-0004-0617-6776}}$, %\IEEEauthorrefmark{1}\IEEEauthorrefmark{2},
Farah Khaled \IEEEauthorrefmark{1}\IEEEauthorrefmark{2}$^{\orcidicon{0009-0001-6869-1288}}$, 
Omar Riad\IEEEauthorrefmark{1}\IEEEauthorrefmark{2}$^{\orcidicon{0009-0007-9128-4158}}$ and
Catherine~M.~Elias$^{\orcidicon{0000-0002-1444-9816}}$,~\IEEEmembership{Member,~IEEE,}\IEEEauthorrefmark{1}\IEEEauthorrefmark{2}
}
\IEEEauthorblockA{
\IEEEauthorrefmark{1}C-DRiVeS Lab: Cognitive Driving Research in Vehicular Systems, Cairo, Egypt\\
Email: cdrives.researchlab@gmail.com
}
\IEEEauthorblockA{
\IEEEauthorrefmark{2}Computer Science and Engineering Department - Faculty of Media Engineering and Technology\\German University in Cairo, Egypt\\
Emails: amrk13415@gmail.com,
farah.abdelghany@student.guc.edu.eg, \\riad.omar2004@gmail.com, catherine.elias@ieee.org
}
}

% make the title area
\maketitle

==> sections/ack.tex <==
\section*{Acknowledgement}


==> sections/authors_bib.tex <==
\newpage
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/gazebo/gaz3.png}}]{Author 1}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Author 2}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{Author 3}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Author 4}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
